Beyond Turn-Based Interfaces: Synchronous LLMs as Full-Duplex Dialogue Agents

Despite broad interest in modeling spoken dialogue agents, most approaches are inherently "half-duplex" -- restricted to turn-based interaction with responses requiring explicit prompting by the user or implicit tracking of interruption or silence events. Human dialogue, by contrast, is "full-duplex" allowing for rich synchronicity in the form of quick and dynamic turn-taking, overlapping speech, and backchanneling. Technically, the challenge of achieving full-duplex dialogue with LLMs lies in modeling synchrony as pre-trained LLMs do not have a sense of "time". To bridge this gap, we propose Synchronous LLMs for full-duplex spoken dialogue modeling. We design a novel mechanism to integrate time information into Llama3-8b so that they run synchronously with the real-world clock. We also introduce a training recipe that uses 212k hours of synthetic spoken dialogue data generated from text dialogue data to create a model that generates meaningful and natural spoken dialogue, with just 2k hours of real-world spoken dialogue data. Synchronous LLMs outperform state-of-the-art in dialogue meaningfulness while maintaining naturalness. Finally, we demonstrate the model's ability to participate in full-duplex dialogue by simulating interaction between two agents trained on different datasets, while considering Internet-scale latencies of up to 240 ms. Webpage: https://syncllm.cs.washington.edu/.

==> human_eval.tex <==
\section{human_eval}



==> interaction.tex <==
\section{Full-duplex voice interaction with SyncLLM}
In the previous section, we show that our Synchronous LLM framework based on auto-regressive transformer decoder architecture is able to generate full-duplex spoken dialogues that are semantically coherent with natural turn-taking ability. Specifically, we observed that our approach is able to leverage extensive text pre-training of auto-regeressive LLMs and transfers the linguistic ability to speech modality, especially in the context of full-duplex dialogue. In this section, we show how Synchornous LLM trained with our 3 stage approach can be used to develop a full-duplex voice interface to the LLM. In Fig. \ref{fig:interaction}, we visualize the voice interaction mechanism between the SyncLLM and user through an audio device. As described in Sec. \xref{sec:training}, in the third and final stage of training, we use spoken dialogue data with individual sides of the conversation recorded in separate audio channels. The speech channels are tokenized, split into chunks and interleaved as shown in Fig. \ref{fig:dedup_model}, where consecutive chunks corresponding to different speakers correspond to same time step. The third training stage then models sequences with these interleaved chunks of tokens, thus giving SyncLLM the ability to predict both sides of the spoken dialogue, chunk by chunk.

The model trained with this approach can be used for full-duplex voice interaction if we could replace one of the two token streams, with that corresponding to the real-world user as shown in the Fig. \ref{fig:interaction}. In Fig. \ref{fig:interaction}, purple boxes correspond to token sequences of LLM's side of the conversation in each time chunk. Similarly, green boxes correspond to user's side of the conversation. As depicted in the figure, we could achieve full-duplex LLM-user voice interaction if we replace the second speaker's side of the conversation with the user's speech -- discarding LLM's predictions of user's response.

\subsection{Latency tolerant interaction.}
\label{sec:latency_tolerant}
Human-to-human voice interactions rely on the ability to model other person's response in the short-term \cite{frontiers}. Specifically, we are capable of taking turns with gaps as small as 200ms, whereas latency required for language generation are close to 600ms. This implies that we anticipate next few words of what the other person would potentially say and respond appropriately. We use these insights in making LLM-User interface latency tolerant. In Fig. \ref{fig:interaction}, consider the Nth time chunk to be current time step. Similar to sequences SyncLLM is trained with in the final stage, we could interleave LLM's output speech chunks until Nth chunk, with user's input chunks corresponding to only N-1 chunks. This is because user's input for the Nth chunk would not available until the end of Nth time step. To handle this instrinsic latency, similar to the way humans anticipate next few words of what other person taking part in the dialogue would say, LLM's output for the next chunk (N+1) is then computed by first estimating User's response for the Nth time chunk (depicted in the figure with green boxes with dotted border). We then append this estimated chunk to the LLM's context to generate LLM's next chunk (N+1). For generating subsequent chunks (N+2, N+3, ...), we discard estimated user's chunk for Nth timestep and replace that with user's real-world input, thus grounding the subsequent interaction with actual input from the user.

\begin{figure}[!t]
\centering
\includegraphics[width=1.0\linewidth]{Figs/two_model_comp.pdf}
\caption{Comparison of ASR perplexity between continuation mode and interaction-mode.}
\label{fig:interaction_comp}
\end{figure}

\begin{figure}[!t]
\centering
\includegraphics[width=1.0\linewidth]{Figs/two_model_latency.pdf}
\caption{Effect of latency on perplexity in two-model interaction setting.}
\label{fig:interaction_latency}
\end{figure}

\begin{table}[!t]
\centering
\caption{Comparison of average Pearson correlation of turn-taking event durations between generation and ground-truth continuation with SyncLLM in the two-model interaction setting. Measured on testsets comprising both Fisher and Candor subsets. [F: SyncLLM trained on Fisher; C: SyncLLM trained on Candor]}
\label{tab:interaction_naturalness}
\begin{tabular}{cccc}
\hline
\textbf{Latency} & \textbf{F <--> F} & \textbf{F <--> C} \\
\hline
160 ms & 0.32 & 0.36 \\
200 ms & 0.31 & 0.35 \\
240 ms & 0.28 & 0.32 \\
\hline
\end{tabular}
\end{table}

\subsection{Evaluation}

To evaluate the full-duplex voice interaction capability, we follow the spoken dialogue evaluation method used in \xref{sec:experiments}. But in contrast to the setting in \xref{sec:experiments}, where LLM generates both sides of the spoken dialogue given a spoken dialogue prompt, here, we evaluate samples obtained by simulating spoken dialogue between two separate instances of the LLM. We use the latency tolerant interaction mechanism described in \xref{sec:latency_tolerant}, to simulate LLM-user interaction using LLM-LLM interaction consider one-chunk latency. We evaluate our model trained with different chunk sizes, thus simulating different amount of latency. Further, we also train a version of SyncLLM with Candor \cite{doi:10.1126/sciadv.adf3197} training split in the third training stage, and simulate its interaction with the original model trained with only Fisher dataset.

To evaluate the semantic coherency of spoken dialogue generated in the two-model interaction setting, similar to \xref{sec:semantic_eval}, we compare perplexities of transcripts of the generated samples. In Fig. \ref{fig:interaction_comp}, we compare median perplexities obtained with prompts sampled from Fisher and Candor test splits. We also show the perplexity of ground-truth and samples generated in the dialog continuation setting for reference. We find that SyncLLM in the LLM-LLM interaction setting is able to closely match the match the performance of the continuation setting, and perform significantly better than dGSLM in continuation setting. Furthermore, we find that interaction between instances of SyncLLM trained with Fisher and Candor datasets, respectively is are almost the same signifying that SyncLLM can perform a coherent conversation even when user's side of the conversation is generated by a model trained with a different dataset.

In Fig. \ref{fig:interaction_latency}, we compare the performance in the interaction setting with different amount of latency. We find that our method is robust to a latency as much as 200 ms, but the performance drops with latency greater than that. Similar to our naturalness evaluation in the continuation setting in \xref{sec:naturalness_eval}, to evaluate turn-taking capability of SyncLLM in interaction setting, we compare Pearson correlation of the duration of turn-taking events in generation and ground-truth continuations. In Table \ref{tab:interaction_naturalness}, we observe that on a combined test set of in-distribution and out-of-distribution prompts, performance in the interaction setting closely match with latencies 160 ms and 200 ms, but drops with 240 ms.

\textcolor{red}{User study results for two-model setting.}


==> method-1.tex <==

\section{SyncLLM}
\label{sec:method}
\begin{figure*}[!t]
\centering
    \begin{subfigure}[c]{0.7\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{Figs/model.pdf}
        \caption{Synchronous dialog language modeling with chunk duration T }
        \label{fig:model}
    \end{subfigure}
    ~
    \begin{subfigure}[c]{0.7\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{Figs/dedup_model.pdf}
        \caption{Synchronous dialog language modeling with deduplicated token sequences and chunk duration T }
        \label{fig:dedup_model}
    \end{subfigure}

    \caption{\hongyu{shall we keep just one of the two subplots? We could add explanations about how (a) and (b) differ to the figure title}}
    \label{fig:method}
\end{figure*}


%Prevailing approach of using cascaded models for spoken dialogue between LLM and an user, ASR → LLM → TTS, assumes a strong correlation with its text representation. But often, users would prefer to speak in informal language with the expectation that the model understands the intent through intonation and turn-taking. We note that in modeling such natural spoken dialogue, the ability to model timing is essential \cite{frontiers, turntake3}. Cascaded approaches using text-only LLMs textual representation of speech, which do not hold information pertaining to either duration of each phoneme in a speech utterance, or the length of silences within or between utterances.


We developed a Transformer decoder-only language model that natively models discrete speech units in a wall-clock synchronous fashion. This results in a language model capable of performing full-duplex spoken dialogue. First, we describe our full-duplex dialogue generation language model and interpret the token sequences it generates. Next, we outline the training process, and finally, we demonstrate how our language model can emulate real-time interaction in the presence of communication latency.

\subsection{Synchronous language model for full-duplex dialogue}
\label{sec:sync_model}

Recent developments in spoken language modeling leverage periodic discrete units to represent speech. Generative spoken language modeling \cite{lakhotia2021generative, kharitonov2022textfree, dgslm}, demonstrate models capable of generating realistic speech, however, due to the lack of large scale speech data combined with low information density of speech compared to text counterparts, these models fail to generate semantically coherent speech. Text-speech multi-modal models such as AudioPALM \cite{rubenstein2023audiopalm} and more recently SpiritLM \cite{nguyen2024spiritlm}, propose to use auto-regressive transformer decoder-only architectures for speech modeling. An advantage with that design decision is that they were able leverage large scale text pre-trained text LLMs, and finetuned them with speech data. This approach results in an LLM capable of natively generating speech, while also retaining semantic capabilities of respective base LLMs.

%To address this, we ask a fundamental question, if language models are run synchronously with the real-world clock while simultaneously modeling both sides of the conversation, could they achieve effective turn-taking, back-channeling etc.? 

While modeling periodic discrete speech units considers timing within the context of an utterance, a crucial missing capability for performing spoken dialogue is the ability to model a common time frame for \emph{both} speakers in the dialogue.  Specifically, as shown in Fig. \ref{fig:sync_w_clock}, we propose that if an LLM's speech is synchronous with a real-world clock, we can achieve synchronization between the LLM's speech and its user's speech.

%The sequence comprises two parallel speech streams interleaved, corresponding to the two speakers.  

To model dialog between two speakers 0 \& 1, we define two special tokens \verb|[S0]| and \verb|[S1]|, referred to as speaker tags, specifying the start of each speaker's token sequence, respectively. The model is trained to generate two speech streams, one for each speaker, interleaved, as shown in the Fig. \ref{fig:model}. For each stream, the model is trained to generate a speaker tag every $T$ seconds, thereby synchronizing with the real-world clock. Thus, the generated token sequence demarcates the progression of time, into \emph{chunks}, each with of duration $T$. Following prior works in spoken language modeling \cite{dgslm, nguyen2024spiritlm}, we use HuBERT \cite{hsu2021hubert} to represent speech tokens. We use the tokenization parameters from \cite{nguyen2024spiritlm}, with a token sampling rate of 25 Hz -- resulting in one token for every 40 ms of audio -- and a vocabulary size of 501. A chunk duration $T = 240 ms$, for instance, would results in $240 ms / 40 ms  = 6$ HuBERT tokens per chunk.



\textbf{Token sequence format and de-duplication.} The fixed time period of HuBERT tokens is beneficial for modeling time in the simultaneous dialog. However, raw HuBERT sequences consist of significant repeated tokens, mainly caused by silence within and across utterances. The number of repetitions of each unique token denote the duration of the acoustic unit represented by the token. The semantic content, however, can be modeling by only considering unique tokens while deduplicating the token sequence \cite{kharitonov2022textfree, dgslm}. Duplicate token sequences have been shown to adversely affect the semantic capability of the final spoken dialogue model \cite{dgslm}, because as shown in Fig. \ref{fig:deduplication}, they contain $\sim50\%$ lower semantic content per token compared to deduplicated token sequences.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{Figs/tokens_per_sec.png}
\caption{Tokens required for representing a second of speech with/without deduplication. Histogram computed over 15 hr of spoken dialog data in Fisher dataset \cite{Cieri2004TheFC}.}
\label{fig:deduplication}
\end{figure}

So, instead, we train the model to predict deduplicated HuBERT sequences, with coarse timing information maintained by periodically interleaved special tokens, \verb|[S0]| and \verb|[S1]|, as shown in  Fig. \ref{fig:dedup_model}. Between two consecutive special tokens of a speaker (a chunk), the model is trained to generate deduplicated HuBERT tokens corresponding to relevant time slots as shown in the Fig. \ref{fig:dedup_model}. Here in the first time chunk, speaker 0's stream contained 2 deduplicated HuBERT tokens \verb|Hu438 & Hu54| and speaker 1's stream contained 1 deduplicated HuBERT token \verb|Hu409|. In the second time slot, speaker 0 has 1 token and speaker 1 has 0 tokens, which means that in the second time slot, speaker 1's stream is just repetition of the token in their first time slot. In the third time slot, both speaker 0 and speaker 1 have 0 deduplicated tokens.

\begin{table*}[!t]
\centering
\caption{Text \& speech dialogues datasets used for training. We convert text-dialogue datasets to spoken dialogue datasets using TTS.}
\label{tab:your_label}
\begin{tabular}{lccc}
\hline
\textbf{Dataset} & \textbf{Stage} & \textbf{Source modality} & \textbf{Total speech duration (hours)} \\
\hline
OpenOrca \cite{OpenOrca} & 1 & Text & 109k \\
Ultrachat \cite{ultrachat} & 1 & Text & 84k \\
\hline
SODA \cite{kim2022soda} & 2 & Text & 19k \\
Prosocial \cite{kim2022prosocialdialog} & 2 & Text & 625 \\
\hline
Fisher \cite{Cieri2004TheFC} & 3 & Speech & 1927 \\
\hline
\end{tabular}
\end{table*}

\subsection{Three-stage training procedure}
\label{sec:training}

Simultaneous spoken dialogue modeling requires speech dialogue data with individual speakers' parts of the conversation separated into different audio streams. This kind of data is available in limited quantities, with the largest resource, the Fisher dataset \cite{Cieri2004TheFC}, comprising   2000 hours. In contrast, text-speech multimodal models require training with over 100,000 hours of speech data \cite{rubenstein2023audiopalm, nguyen2024spiritlm}. 

In the dGSLM study \cite{dgslm}, which was exclusively trained on the Fisher dataset, it was observed that while conversation cues were effectively learned, it failed to generate semantically coherent speech. To address this, we  instead chose a transformer decoder-only architecture. We utilized the large-scale pre-trained LLM, Llama3 \cite{llama3}, as our base model and performed three rounds of fine-tuning to gradually develop our full-duplex dialogue model.


\textbf{Stage 1: Turn-based spoken dialogue model with synthetic speech data.} Since our base model is a text-only LLM, in the first stage of finetuning we train the base model to be a turn-based spoken dialogue. Given a spoken question, in this stage we train the model to generate a spoken response. We first expand the vocabulary of Llama3 to include 501 HuBERT tokens, in addition to the speaker tags, \verb|[S0]| and \verb|[S1]|. A turn-based dialog could be defined as made of turns, which in turn are made of sentences. We finetuned Llama3 with dialog sequences in the following format:
\begin{verbatim}
[S1]<sent0>[S0]<sent0><sent1>[S1]..
\end{verbatim}
Here, each sentence is randomly chosen to either be text or fully deduplicated speech token sequences during training. This sentence level text-speech interleaving method not only trains the model to be capable of performing dialog, but also achieves text/speech alignment in the context of dialog. 

Given the limited spoken dialogue data, we generate synthetic speech  data based on large-scale text dialog datasets. We use open-source supervised finetuning (SFT) datasets OpenOrca \cite{OpenOrca} \& Ultrachat \cite{ultrachat}, as our source text-dialogue datasets. We used Bark TTS \cite{barktts} model to generate spoken versions of text-dialogue datasets, with 10 speaker presets that are available with the Bark TTS model.

\textbf{Stage 2: Simulataneous dialogue model assuming no overlaps.} Turn-based spoken dialogue is special case of simulataenous dialogue with no overlaps. Based on this observation, we could treat synthetic spoken dialogue data as simultaneous spoken dialogue data where during one speaker's turn, other speaker is completely silent. In this stage, we create synthetic spoken dialogue data from text-dialogue data similarly to the previous stage with one main difference: From each turn in the dialogue, we generate a speech uttereance corresponding to one speaker and silence of equal duration corresponding to the other speaker. We then tokenize the parallel speech dialog data, deduplicate with time synchronized speaker tag embedded in the sequence. This way, we can further leverage text-dialogue data for training our model to generate simulataneous dialogue in the token sequence format described in \xref{sec:sync_model}. This stage of finetuning models timing within an utterance. The model cannot learn turn-taking cues such as back-channeling or overlaps between two speaker yet. For this stage, we use SODA \cite{kim2022soda} and Prosocial-dialog \cite{kim2022prosocialdialog} as our source text-dialogue datasets, which resulted in around $10$k hrs of synthetic spoken dialogue data.

This approach of modeling simulatenous dialogue with syncthetic data is technically applicable to SFT datasets we used in the previous stage. However, in SFT datasets, most samples would contain one speaker (user of the LLM) taking a short turn and the other speaker (the LLM) giving a long response. This resulted in long silences for one of speakers and disproportionately large number of speaker tags compared to HuBERT tokens, causing training instability. We observed that finetuning the base text-only LLM with deduplicated speech utterances, and then introducing time synchronized speaker tags, results in stable training.


\begin{table*}[!t]
\centering
\caption{Comparison of Pearson correlation of turn-taking event durations between prompt and generation.}
\label{tab:model_performance}
\begin{tabular}{l*{4}{c}c*{4}{c}}
\hline
\textbf{Model} & \multicolumn{4}{c}{\textbf{Fisher (in-distribution)}} & \phantom{|} & \multicolumn{4}{c}{\textbf{Candor (out-of-distribution)}} \\
\cline{2-5} \cline{7-10}
& \textbf{ipu} & \textbf{pause} & \textbf{fto} & \textbf{Average} && \textbf{ipu} & \textbf{pause} & \textbf{fto} & \textbf{Average} \\
\hline
dGSLM & 0.60 & 0.34 & 0.23 & 0.39 && 0.43 & 0.20 & 0.09 & 0.24 \\
SyncLLM (160 ms) & 0.69 & 0.34 & 0.35 & 0.46 && 0.64 & 0.12 & 0.24 & 0.33 \\
SyncLLM (200 ms) & 0.57 & 0.49 & 0.29 & 0.45 && 0.61 & 0.34 & 0.13 & 0.36 \\
SyncLLM (240 ms) & 0.63 & 0.49 & 0.33 & 0.48 && 0.59 & 0.23 & 0.19 & 0.34 \\
\hline
GT & 0.72 & 0.53 & 0.31 & 0.52 && 0.54 & 0.30 & 0.12 & 0.32 \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[!t]
\centering
\caption{Comparison of Pearson correlation of turn-taking event durations between generations and ground-truth continuations, given same prompts. \textcolor{red}{Alternative to prompt <--> generation correlation.}}
\label{tab:model_performance}
\begin{tabular}{l*{4}{c}c*{4}{c}}
\hline
\textbf{Model} & \multicolumn{4}{c}{\textbf{Fisher (in-distribution)}} & \phantom{|} & \multicolumn{4}{c}{\textbf{Candor (out-of-distribution)}} \\
\cline{2-5} \cline{7-10}
& \textbf{ipu} & \textbf{pause} & \textbf{fto} & \textbf{Average} && \textbf{ipu} & \textbf{pause} & \textbf{fto} & \textbf{Average} \\
\hline
dGSLM & 0.48 & 0.41 & 0.10 & 0.33 && 0.30 & 0.02 & 0.09 & 0.14 \\
SyncLLM (160 ms) & 0.60 & 0.50 & 0.20 & 0.43 && 0.45 & 0.09 & 0.14 & 0.23 \\
SyncLLM (200 ms) & 0.60 & 0.49 & 0.19 & 0.43 && 0.44 & 0.28 & 0.14 & 0.29 \\
SyncLLM (240 ms) & 0.58 & 0.40 & 0.25 & 0.41 && 0.45 & 0.27 & 0.21 & 0.31 \\
\hline
Prompt & 0.72 & 0.53 & 0.31 & 0.52 && 0.54 & 0.30 & 0.12 & 0.32 \\
Resynth-GT & 0.92 & 0.92 & 0.53 & 0.79 && 0.90 & 0.86 & 0.37 & 0.71 \\
\hline
\end{tabular}
\end{table*}

\textbf{Stage 3: Simulataneous dialogue model.} Finally, we fine-train the model to learn turn-taking cues from real-world spoken dialogue data. We use the Fisher \cite{Cieri2004TheFC} dataset with  2000 hours of spoken dialogues, where each speaker's speech in a dialogue is separated into independent audio channels. Each audio channel in the dialogue is separately tokenized and interleaved in the full-duplex dialogue format used in the previous stage. With real-world spoken dialogue data however, the model learns conversational cues like accurate distribution of pauses between turn and backchanneling.

% \subsection{Latency-tolerant real-time interaction}


==> method.tex <==

\section{Method}
\begin{figure*}[!t]
\centering
    \begin{subfigure}[c]{0.7\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{Figs/model.pdf}
        \caption{Synchronous dialog language modeling with chunk duration T }
        \label{fig:model}
    \end{subfigure}
    ~
    \begin{subfigure}[c]{0.7\linewidth}
        \centering
        \includegraphics[width=1.0\linewidth]{Figs/dedup_model.pdf}
        \caption{Synchronous dialog language modeling with deduplicated token sequences and chunk duration T }
        \label{fig:dedup_model}
    \end{subfigure}

    \caption{}
    \label{fig:method}
\end{figure*}


Prevailing approach of using cascaded models for spoken dialogue between LLM and an user, ASR → LLM → TTS, assumes a strong correlation with its text representation. But often, users would prefer to speak in informal language with the expectation that the model understands the intent through intonation and turn-taking. We note that in modeling such natural spoken dialogue, the ability to model timing is essential \cite{frontiers, turntake3}. Cascaded approaches using text-only LLMs textual representation of speech, which do not hold information pertaining to either duration of each phoneme in a speech utterance, or the length of silences within or between utterances.

Recent developments in spoken language modeling leverage periodic discrete units to represent speech. Generative spoken language modeling \cite{lakhotia2021generative, kharitonov2022textfree, dgslm}, demonstrate models capable of generating realistic speech, however, due to the lack of large scale speech data combined with low information density of speech compared to text counterparts, these models fail to generate semantically coherent speech. Text-speech multi-modal models such as AudioPALM \cite{rubenstein2023audiopalm} and more recently SpiritLM \cite{nguyen2024spiritlm}, propose to use auto-regressive transformer decoder-only architectures for speech modeling. An advantage with that design decision is that they were able leverage large scale text pre-trained text LLMs, and finetuned them with speech data. This approach results in an LLM capable of natively generating speech, while also retaining semantic capabilities of respective base LLMs.

Considering these aspects, we develop an multi-modal transformer decoder-only LLM, SyncLLM, that natively models discrete speech units in wall-clock synchronous fashion, resulting in a model capable of performing simultaneous spoken dialogue. We first describe our simultaneous dialogue generation LLM and the interpretation of token sequences it generates. We then describe the training recipe and finally, show how our LLMs can emulate a real-time interaction in the presence of communication latency.

\subsection{Synchronous language model for full-duplex dialogue}
\label{sec:sync_model}

While modeling with periodic discrete speech units consider timing within the context of an utterance, a key capability that is still missing but important for performing spoken dialogue is the ability to model a common time-frame for \emph{both} speakers in the dialogue. To address this, we ask a fundamental question, if language models are run synchronously with the real-world clock while simultaneously modeling both sides of the conversation, could they achieve effective turn-taking, back-channeling etc.? As shown in Fig. \ref{fig:sync_w_clock}, we propose that if an LLM's speech is synchronous with a real-world clock, we can achieve synchronization between LLM's speech with its user's speech.

To model dialog between two speakers 0 \& 1, we define two special tokens \verb|[S0]| and \verb|[S1]|, referred to as speaker tags, specifying the start of each speaker's token sequence, respectively. The model is trained to generate two speech streams one for each speaker, interleaved, as shown in the Fig. \ref{fig:model}. The sequence comprises two parallel speech streams interleaved, corresponding to speaker 0 and speaker 1. For each stream, the model is trained to generate a speaker tag every $T$, thereby synchronized in time. Thus the generated token sequence demarcates the progression of time, into \emph{chunks}, each with of duration $T$. Following prior works in spoken language modeling \cite{dgslm, nguyen2024spiritlm}, we use HuBERT \cite{hsu2021hubert} tokens to represent speech. We use the tokenization parameters used in \cite{nguyen2024spiritlm}, with a token sampling rate of 25 Hz -- resulting in one token for every 40 ms of audio -- and a vocabulary size of 501. A chunk duration $T = 240 ms$, for instance, would results in $240 ms / 40 ms  = 6$ HuBERT tokens per chunk.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{Figs/tokens_per_sec.png}
\caption{Tokens required for representing a second of speech with/without deduplication. Histogram computed over 15 hr of spoken dialog data in Fisher dataset \cite{Cieri2004TheFC}.}
\label{fig:deduplication}
\end{figure}

\textbf{Token sequence format.} The fixed time period of HuBERT tokens is beneficial for modeling time in the simultaneous dialog. However, raw HuBERT sequences consist of significant repeated tokens, mainly caused by silence within and across utterances. The number of repetitions of each unique token denote the duration of the acoustic unit represented by the token. The semantic content, however, can be modeling by only considering unique tokens while deduplicating the token sequence \cite{kharitonov2022textfree, dgslm}. Duplicate token sequences have been shown to adversely affect the semantic capability of the final spoken dialogue model \cite{dgslm}, because as shown in Fig. \ref{fig:deduplication}, contains $\sim50\%$ lower semantic content per token compared to deduplicated token sequences.

So, instead, we train the model to predict deduplicated HuBERT sequences, with coarse timing information maintained by periodically interleaved special tokens \verb|[S0]| and \verb|[S1]|, as shown in the Fig. \ref{fig:dedup_model}. Between two consecutive special tokens of a speaker (a chunk), the model is trained to generate deduplicated HuBERT tokens corresponding to relevant time slots as shown in the Fig. \ref{fig:dedup_model}. Here in the first time chunk, speaker 0's stream contained 2 deduplicated HuBERT tokens \verb|Hu438 & Hu54| and speaker 1's stream contained 1 deduplicated HuBERT token \verb|Hu409|. In the second time slot, speaker 0 has 1 token and speaker 1 has 0 tokens, which means that in the second time slot, speaker 1's stream is just repetition of the token in their first time slot. In the third time slot, both speaker 0 and speaker 1 have 0 deduplicated tokens.

\begin{table*}[!t]
\centering
\caption{Text \& speech dialogues datasets used for training. We convert text-dialogue datasets to spoken dialogue datasets using TTS.}
\label{tab:your_label}
\begin{tabular}{lccc}
\hline
\textbf{Dataset} & \textbf{Stage} & \textbf{Source modality} & \textbf{Total speech duration (hours)} \\
\hline
OpenOrca \cite{OpenOrca} & 1 & Text & 109k \\
Ultrachat \cite{ultrachat} & 1 & Text & 84k \\
\hline
SODA \cite{kim2022soda} & 2 & Text & 19k \\
Prosocial \cite{kim2022prosocialdialog} & 2 & Text & 625 \\
\hline
Fisher \cite{Cieri2004TheFC} & 3 & Speech & 1927 \\
\hline
\end{tabular}
\end{table*}

\subsection{Training}

Simultaneous spoken dialogue modeling requires speech dialogue data with individual speaker's part of the conversation separated into different audio streams. This kind of data available in limited quantities with the largest available resource, Fisher  dataset \cite{Cieri2004TheFC}, being 2000 hrs in size. To put this in perspective, text-speech multimodal models require training with > 100k hours of speech \cite{rubenstein2023audiopalm, nguyen2024spiritlm}. Here, we note the result observed in dGSLM \cite{dgslm}, which is exclusively trained on the Fisher dataset. dGSLM observed that while conversation cues are effectively learnt with available spoken dialog data, it fails to generate semantically coherent speech. Our choice of transformer decoder-only architecture is primarily to address this challenge. We use a large-scale pre-trained LLM, Llama3 \cite{llama3}, as our base model and perform three rounds of finetuning to gradually obtain the simultaneous dialogue model described in \xref{sec:sync_model}.

\textbf{Stage 1: Turn-based spoken dialogue model.} Since our base model is a text-only LLM, in the first stage of finetuning we train the base model to be a turn-based spoken dialogue. Given a spoken question, in this stage we train the model to generate a spoken response. We first expand the vocabulary of Llama3 to include 501 HuBERT tokens, in addition to the speaker tags, \verb|[S0]| and \verb|[S1]|. A turn-based dialog could be defined as made of turns, which in turn are made of sentences. We finetuned Llama3 with dialog sequences in the following format:
\begin{verbatim}
[S1]<sent0>[S0]<sent0><sent1>[S1]..
\end{verbatim}

where each sentence is randomly chosen to either be text or fully deduplicated speech token sequences during training. This sentence level text-speech interleaving method not only trains the model to be capable of performing dialog, but also achieves text/speech alignment in the context of dialog.

Given the limited spoken dialogue data, we generate synthetic spoken dialogue data based on large-scale text dialog datasets. We use open-source supervised finetuning (SFT) datasets OpenOrca \cite{OpenOrca} \& Ultrachat \cite{ultrachat}, as our source text-dialogue datasets. We used Bark TTS \cite{barktts} model to generate spoken versions of text-dialogue datasets, with 10 speaker presets that are available with the Bark TTS model.

\textbf{Stage 2: Simulataneous dialogue model assuming no overlaps.} Turn-based spoken dialogue is special case of simulataenous dialogue with no overlaps. Based on this observation, we could treat synthetic spoken dialogue data as simultaneous spoken dialogue data where during one speaker's turn, other speaker is completely silent. In this stage, we create synthetic spoken dialogue data from text-dialogue data similarly to the previous stage with one main difference: From each turn in the dialogue, we generate a speech uttereance corresponding to one speaker and silence of equal duration corresponding to the other speaker. We then tokenize the parallel speech dialog data, deduplicate with time synchronized speaker tag embedded in the sequence. This way, we can further leverage text-dialogue data for training our model to generate simulataneous dialogue in the token sequence format described in \xref{sec:sync_model}. This stage of finetuning models timing within an utterance. The model cannot learn turn-taking cues such as back-channeling or overlaps between two speaker yet, though. For this stage we use SODA \cite{kim2022soda} \& Prosocial-dialog \cite{kim2022prosocialdialog} as our source text-dialogue datasets, which resulted in $~10$k hrs of synthetic spoken dialogue data.

This approach of modeling simulatenous dialogue with syncthetic data is technically applicable to SFT datasets we used in the previous stage. However, in SFT datasets, most samples would contain one speaker (user of the LLM) taking a short turn and the other speaker (the LLM) giving a long response. This resulted in long silences for one of speakers and disproportionately large number of speaker tags compared to HuBERT tokens, causing training instability. We observed that finetuning the base text-only LLM with deduplicated speech utterances, and then introducing time synchronized speaker tags, results in stable training.


\begin{table*}[!t]
\centering
\caption{Comparison of Spearman correlation of turn-taking event durations between prompt and generation.}
\label{tab:model_performance}
\begin{tabular}{l*{4}{c}c*{4}{c}}
\hline
\textbf{Model} & \multicolumn{4}{c}{\textbf{Fisher (in-distribution)}} & \phantom{|} & \multicolumn{4}{c}{\textbf{Candor (out-of-distribution)}} \\
\cline{2-5} \cline{7-10}
& \textbf{ipu} & \textbf{pause} & \textbf{fto} & \textbf{Average} && \textbf{ipu} & \textbf{pause} & \textbf{fto} & \textbf{Average} \\
\hline
DGSLM & 0.55 & 0.35 & 0.26 & 0.39 && 0.45 & 0.18 & 0.16 & 0.26 \\
SyncLLM (160 ms) & 0.68 & 0.35 & 0.32 & \textbf{0.45} && 0.61 & 0.19 & 0.20 & 0.33 \\
SyncLLM (200 ms) & 0.58 & 0.46 & 0.25 & 0.43 && 0.63 & 0.30 & 0.19 & \textbf{0.37} \\
SyncLLM (240 ms) & 0.63 & 0.45 & 0.21 & 0.43 && 0.59 & 0.28 & 0.22 & 0.36 \\
\hline
Reference & 0.67 & 0.50 & 0.28 & 0.48 && 0.57 & 0.30 & 0.19 & 0.35 \\
\hline
\end{tabular}
\end{table*}

\textbf{Stage 3: Simulataneous dialogue model.} In the final stage of finetuning, we train the model to learn turn-taking cues from real-world spoken dialogue data. We use the Fisher \cite{Cieri2004TheFC} dataset comprising of 2000 hours of spoken dialogues, where each speaker's speech in a dialogue is separated into independent audio channels. Each audio channel in the dialogue is separately tokenized and interleaved in the full-duplex dialogue format used in the previous stage. With real-world spoken dialogue data however, the model learns accurate distribution of pauses between turn, to backchannel and so on.

% \subsection{Latency-tolerant real-time interaction}


==> related.tex <==
\section{Related work}

% multimodal LM
\textbf{Multimodal language model}. The success of text language models such as GPT-4 \cite{gpt4}, \textsc{Llama} \cite{llama2} and Mistral \cite{mistral} have inspired explorations into multimodal models. In this work we focus our discussion on speech and text modalities. It has been found that initialization from a pretrained text LLM benefits the multimodal training \cite{textually_pretrain}. Recent works proposed to extend the vocabulary of text LLM with discrete speech tokens to enable the model to handle speech inputs and outputs \cite{rubenstein2023audiopalm}. Models are trained with cross-modal knowledge from aligned speech-text data such as automatic speech recognition (ASR), text-to-speech synthesis (TTS), speech-to-text (S2T) and speech-to-speech (S2ST). Multitask learning with these tasks are adopted by VioLA \cite{viola}, AudioPaLM \cite{rubenstein2023audiopalm}, VoxtLM \cite{voxtlm} and SUTLM \cite{sutlm}. SpiRit-LM \cite{nguyen2024spiritlm} interleaves speech and text tokens and trains the model with next token prediction, demonstrating speech understanding and generation. 

% AudioPaLM \cite{rubenstein2023audiopalm}: init from text LLM, speech understanding and generation. 
% SpiRit-LM \cite{nguyen2024spiritlm}: init from text LLM, speech understanding and generation.
% VioLA  multitask learning for speech recognition, text-to-speech and text translation, trained from scratch
% : init from pretrained llm, speech recognition, synthesis, text generation, speech continuation.
% jointly trains speech and text LMs on ASR, TTS and speech/text continuation.
% TWIST \cite{textually_pretrain} train speechLM with warm-start from pretraied text LM \textsc{Llama} for spoken language understanding and speech generation.


% dialogue/conversation

\textbf{Spoken dialogue model}. There is a long line of dialogue research covering various topics such as dialogue state tracking \cite{monet}, turn-taking prediction \cite{turn_taking} and response generation \cite{chatbot}. Recent works leverage LLM in the dialogue system \cite{dialogue_gen}. Initialized from \textsc{Llama}, SpeechGPT \cite{speechgpt} is finetuned sequentially on speech-only data and multimodal instruction sets to perform spoken question answering (QA) task. USDM \cite{USDM} continues pretraining Mistral with interleaved speech-text data to capture multimodal semantics. As for dialogue finetuning, it constructs the template with both speech and transcripts of user input as instruction data. Different from modeling speech tokens, Spectron \cite{spectron} directly manipulates spectrograms for the task of spoken QA and speech continuation.

Despite the improved dialogue quality, these works are mostly limited to turn-taking setting, where the dialogue model is explicitly prompted to speak in its own turn. Human spoken dialogue is more complicated in implicit turn-taking cues, and overlapping speech such as interruptions and backchanneling could happen \cite{schegloff2000overlapping}.

One most relevant work to our study is dGSLM \cite{lakhotia2021generative}, modeling simultaneous dialogue with a dual-tower Transformer architecture. Each tower models one interlocutor, and it can communicate with the other tower by attending to its hidden states via cross-attention. One weakness of dGSLM is the speech-only training, which does not make full use of textual knowledge. This work takes advantage of generative intelligence of language model and equips it with multimodal and synchronous capability. \hongyu{Moreover, dGSLM has not considered delays in real-life scenarios by simply assuming that hidden states of one interlocutor could be immediately accessible to the other. In this study, we discussed how our model handles delayed responses in dialogue.
}






% turn-taking.
% architecture: cascaded, end-to-end



==> results.tex <==

\section{Experiments}
\label{sec:experiments}

Similar to \cite{dgslm}, we evaluate the SyncLLM on semantics and naturalness of generated conversation. We first show the performance of our model on a set of spoken dialogue prompts in our test set, using automatic metrics. We then discuss results from a qualitative evaluation of the dialog generations by our model in a user study. For automatic metrics, we consider prompts from test splits of in-distribution dataset Fisher \cite{Cieri2004TheFC}, as well as an out-of-distribution dataset Candor \cite{doi:10.1126/sciadv.adf3197}.

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{Figs/continuation_comp.pdf}
\caption{Comparison of ASR perplexity with respect to DialoGPT \cite{zhang2019dialogpt}. \textcolor{red}{TODO: Update caption.}}
\label{fig:cont_comp}
\end{figure}

\begin{figure}[h]
\centering
\includegraphics[width=1.0\linewidth]{Figs/continuation_ood.pdf}
\caption{Comparison of in-distribution and out-of-distribution perplexity. \textcolor{red}{TODO: Update legend.}}
\label{fig:cont_ood}
\end{figure}


\subsection{Semantic evaluation}
\label{sec:semantic_eval}
We evaluate the semantics of SyncLLM in the text domain by converting spoken generations to text using Whisper's \cite{radford2022robust} implementation in the WhisperX framework \cite{bain2022whisperx}. We transcribe the generated spoken dialogues into turn-based text dialogues ignoring any overlapping speech. Following \cite{dgslm}, we then use DialoGPT \cite{zhang2019dialogpt} to compute perplexity of transcribed dialogues generated with 10 second spoken dialogue prompts. To account for outliers (samples with abnormally high perplexities), we consider median perplexity over the testset for semantic evaluation. We observed that DailoGPT correlates well with the transcribed spoken dialogue for $\sim$30 seconds of ground-truth continuation -- ground-truth continuation results in 20-30 median perplexity. However, the median perplexity of 40s or longer ground-truth continuation exceeds 50. Considering higher alignment between ground-truth and DialoGPT's predictions, we evaluate the meaningfulness of different models by comparing perplexity of transcripts corresponding to 30s spoken dialogue generations, with respect of DialoGPT model.

In Fig. \ref{fig:cont_comp}, we compare the semantic quality of spoken dialogues generated by SyncLLM models (with different chunk sizes) to the generations by state-of-the-art full-duplex model dGSLM \cite{dgslm} and ground-truth continuations. We find that transcriptions of spoken dialogue generations by dGSLM result in perplexity drop of $\sim$70 relative to the ground-truth, whereas our method only results in a drop of $\sim$15. We compare median perplexities measured with prompts sampled from Fisher and Candor test splits separately, with all models trained only on Fisher training split. So for this evaluation Candor test split is an out-of-distribution testset. We observe in Fig. \ref{fig:cont_ood} that our method is more robust to distribution shift compared to the state-of-the-art dGSLM.

These evaluations show that our approach of using the standard auto-regressive architecture, thus leveraging vast text pre-training, results in much more semantically coherent spoken dialogue model, compared to a custom architecture proposed for speech-only training. Furthermore, our three-stage training approach leveraging large amount of synthetic spoken dialogue data generated from text dialogues, allows us to converge much faster on limited real-world dual-channel spoken dialogue data. This results in a general model that has superior out-of-distribution performance.

\subsection{Naturalness evaluation}
\label{sec:naturalness_eval}
For semantic evaluation, we ignore timing and overlaps of speech between the two speakers. This allowed us to compare the generations with predictions of turn-based text dialogues models. However, appropriate timing of pauses, speaker transitions and overlaps are integral part of spoken-dialogue which convey essential information required for natural spoken conversation. To evaluate these aspect of our generated spoken dialogues, we consider the turn-taking metrics proposed in \cite{dgslm} that evaluate overall naturalness of generated spoken dialogues: inter-pausal units (IPUs), silences, overlaps and floor-transfer offset (fto).

We follow dGSLM's setup of using 30s prompts sampled from the test splits and computing a pair-wise correlation of turn-taking event durations between the prompts and spoken dialogue generations with those prompts. We first compute voice activities of each side of dialogue (generated in each audio channel) usind the voice-activty detector in the \verb|pyannote.audio| library \cite{Bredin2020}. We then use the turn-taking event definitions used in dGSLM to compute start and end timestamps for each turn-taking event occurring in generated spoken dialogues. In Table \ref{tab:model_performance}, we measure the average duration of the turn-taking events in each generated dialogue and then compute Pearson correlation between the average durations observed in the prompt and those in the generation, for each turn-taking event.

Similar to semantic evaluation in Fig. \ref{fig:cont_ood}, we compare turn-taking event correlation between prompt and generations with in-distribution Fisher \cite{Cieri2004TheFC} test-split and out-of-distribution Candor test-split. We observe that, similar to the baseline dGSLM, generations with our models achieve correlation similar to what the ground-truth achieves on both in-distribution and out-of-distribution testsets.

\subsection{Human Evaluation}
In addition to the evaluation with automatic metrics, we also conducted an extensive user study with $n_p=32$ participants subjectively evaluating the generated spoken dialogues. Participants evaluated the generations by providing their opinion scores on both naturalness and meaningfulness of generated dialogues. We collected the mean-opinion scores (MOS) over 90 1-minute generations obtained with 30s prompts. Following \cite{dgslm}, we collected MOS on both naturalness, denoted by N-MOS, and meaningfulness denoted by M-MOS.

\subsubsection{N-MOS and M-MOS}
We adapt the Mean Opinion Score (MOS) protocol (a 5-pt Likert scale) \cite{p808} to evaluate the naturalness of the turn-taking and meaningfulness of the dialogue content. For both N-MOS and M-MOS annotators are presented with the prompt audio and the continuation audio. 

In total $n_{annot}=32$ annotators provided ratings for $n=180$ items divided evenly between the CANDOR and Fisher datasets. Each sample receives a rating from $1 - Bad, ..., 5 - Excellent$ by three unique raters. Annotators are asked to first listen the prompt audio, then the continuation audio. For each pair they provide a rating of the \textit{naturalness} of the continuation as well as the \textit{meaningfulness} (guidelines are presented in full in XYZ location).

We compute item-level scores by taking the median score per item. To compute system-level scores we take the mean of item scores for a given system. We compute 95\% confidence intervals via bootstrapping, resampling the item level for $n_b=1000$ iterations.

% \begin{table}[htbp!]
\begin{table*}[!t]
\centering
% \small
\begin{tabular}{rcccccc}
\toprule
 & \multicolumn{2}{c}{\textbf{Overall}} & \multicolumn{2}{c}{\textbf{Fisher}}  & \multicolumn{2}{c}{\textbf{CANDOR}}\\ 
\cmidrule(rr){2-3}\cmidrule(rr){4-5}\cmidrule(rr){6-7}
\textbf{Model} & Meaning. $\uparrow$ & Nat. $\uparrow$ & Meaning. $\uparrow$ & Nat. $\uparrow$ & Meaning. $\uparrow$ & Nat. $\uparrow$ \\
\midrule
dGSLM & 1.55 (0.06) & 3.95 (0.08) & 1.67 (0.09) & 4.21 (0.08) & 1.43 (0.08) & 3.70 (0.12) \\
SyncLLM-C & 3.40 (0.07) & 3.96 (0.06) & 3.14 (0.10) & 3.97 (0.08) & 3.66 (0.08) & 3.94 (0.08) \\
SyncLLM-F & 3.74 (0.06) & 3.90 (0.06) & 3.82 (0.08) & 3.98 (0.08) & 3.67 (0.09) & 3.82 (0.10) \\
Re-synth & 3.87 (0.06) & 4.03 (0.05) & 4.04 (0.08) & 4.14 (0.08) & 3.69 (0.07) & 3.91 (0.06) \\
\hline
GT & 4.96 (0.02) & 4.96 (0.02) & 4.96 (0.03) & 4.94 (0.04) & 4.97 (0.02) & 4.98 (0.02) \\
\bottomrule
\end{tabular}
\caption{Human evaluation results for Meaningfulness (Meaning.) and Naturalness (Nat.) mean estimates and standard errors (in parentheses), aggregated overall and for Fisher (in-distribution) and CANDOR (out-of-distribution) subsets.}
\label{tab:human_eval_overall}
\end{table*}

% Keep
% \begin{table*}[!t]
% \label{tab:nmos_mmos_overall}
% \begin{tabular}{r|cc}
% \hline
% Model & N-MOS & M-MOS \\
% \midrule
% dGSLM & 3.95 (0.07) & 1.55 (0.06) \\
% CANDOR & 3.96 (0.05) & 3.40 (0.07)  \\
% Fisher & 3.90 (0.06) & 3.74 (0.06) \\
% Resynth & 4.03 (0.05) & 3.87 (0.06) \\
% \hline
% GT & 4.96 (0.02) & 4.96 (0.02)
% % \hline
% % \label{tab:human_eval_overall}
% \end{tabular}
% \caption{Mean and bootstrap sampled standard errors (in parentheses) aggregated across Fisher and CANDOR datasets.}
% \end{table*}

\textbf{Overall results} (two left-most columns of Table \ref{tab:human_eval_overall}) indicate that nearly all models are at parity in perceived naturalness, however still significantly below ground-truth continuations, which are at ceiling. On the perceived meaningfulness of the dialogues, however, SyncLLM significantly outperforms dGSLM, approaching re-synthesized ground-truth values.
% \footnote{
% 5 - \textit{Excellent - basically indistinguishable from human-like turn-taking}\\
% 4 - \textit{Good - minor differences from human-like turn-taking}
% 3 - \textit{Fair - substantial differences from human-like turn-taking}
% 2 - \textit{Poor - very little in common with human-like turn-taking}
% 1 - \textit{Bad - essentially nothing in common with human-like turn-taking}} 

\textbf{In-domain and OOD} We also include results broken down by in-domain (Fisher) and out-of-domain (OOD) (CANDOR) subset. Of particular interest is the difference between in-distribution and OOD between dGSLM and Fisher-trained SyncLLM-F. While dGSLM suffers from significant degradation OOD (dropping -0.24 and -0.51 in meaningfulness and naturalness ratings), these declines are reduced in SyncLLM-F only dropping -0.15 and -0.16 moving OOD. SyncLLM trained on CANDOR dataset (SyncLLM-C) shows a significant decline OOD on meaningfulness (-0.52), but not naturalness (+0.03). Deeper analysis into this findings is beyond the scope of this paper as it would ideally consider whether a similar effect is found for dGSLM.

% \textbf{Model} & \multicolumn{4}{c}{\textbf{Fisher (in-distribution)}} & \phantom{|} & \multicolumn{4}{c}{\textbf{Candor (out-of-distribution)}} \\
% \cline{2-5} \cline{7-10}
% & \textbf{ipu} & \textbf{pause} & \textbf{fto} & \textbf{Average} && \textbf{ipu} & \textbf{pause} & \textbf{fto} & \textbf{Average} \\
% \hline
% dGSLM & 0.48 & 0.41 & 0.10 & 0.33 && 0.30 & 0.02 & 0.09 & 0.14 \\
% SyncLLM (160 ms) & 0.60 & 0.50 & 0.20 & 0.43 && 0.45 & 0.09 & 0.14 & 0.23 \\
% SyncLLM (200 ms) & 0.60 & 0.49 & 0.19 & 0.43 && 0.44 & 0.28 & 0.14 & 0.29 \\
% SyncLLM (240 ms) & 0.58 & 0.40 & 0.25 & 0.41 && 0.45 & 0.27 & 0.21 & 0.31 \\
% \hline
% Prompt & 0.72 & 0.53 & 0.31 & 0.52 && 0.54 & 0.30 & 0.12 & 0.32 \\
% Resynth-GT & 0.92 & 0.92 & 0.53 & 0.79 && 0.90 & 0.86 & 0.37 & 0.71 \\
% \hline



% \subsection{Ablations}


